Joint Initial Access and Localization in Millimeter Wave Vehicular Networks: a Hybrid Model/Data Driven Approach

High resolution compressive channel estimation provides information for vehicle localization when a hybrid mmWave MIMO system is considered. Complexity and memory requirements can, however, become a bottleneck when high accuracy localization is required. An additional challenge is the need of path order information to apply the appropriate geometric relationships between the channel path parameters and the vehicle, RSU and scatterers position. In this paper, we propose a low complexity channel estimation strategy of the angle of departure and time difference of arrival based on multidimensional orthogonal matching pursuit. We also design a deep neural network that predicts the order of the channel paths so only the LoS and first order reflections are used for localization. Simulation results obtained with realistic vehicular channels generated by ray tracing show that sub-meter accuracy can be achieved for 50% of the users, without resorting to perfect synchronization assumptions or unfeasible all-digital high resolution MIMO architectures.

==> Machine Learning Aided mmWave Vehicular Localization/Other/acronyms.tex <==
\DeclareAcronym{3GPP}{
  short=3GPP,
  long=3rd generation partnership project
}
\DeclareAcronym{5G}{
  short=5G,
  long=fifth-generation
}
\DeclareAcronym{ADC}{
  short=ADC,
  long=analog-to-digital converter
}
\DeclareAcronym{AMP}{
  short=AMP,
  long=approximate message passing
}
\DeclareAcronym{AoA}{
  short=AoA,
  long=angle-of-arrival
}
\DeclareAcronym{AoD}{
  short=AoD,
  long=angle-of-departure
}
\DeclareAcronym{APS}{
  short=APS,
  long=azimuth power spectrum
}
\DeclareAcronym{AV}{
  short=AV,
  long=autonomous vehicle
}
\DeclareAcronym{BS}{
  short=BS,
  long=base station
}
\DeclareAcronym{BSM}{
  short=BSM,
  long=basic safety message
}
\DeclareAcronym{CDF}{
	short=CDF,
	long=cumulative distribution function
}
\DeclareAcronym{CP}{
  short=CP,
  long=cyclic-prefix
}
\DeclareAcronym{DFT}{
  short=DFT,
  long=discrete Fourier transform
}
\DeclareAcronym{DL}{
  short=DL,
  long=downlink
}
\DeclareAcronym{DNN}{
  short=DNN,
  long=deep neural network
}
\DeclareAcronym{DSRC}{
  short=DSRC,
  long=dedicated short-range communication
}
\DeclareAcronym{FC}{
  short=FC,
  long=fully connected
}
\DeclareAcronym{FDD}{
  short=FDD,
  long=frequency division duplex
}
\DeclareAcronym{FMCW}{
  short=FMCW,
  long=frequency modulated continuous wave
}
\DeclareAcronym{FoV}{
  short=FoV,
  long=field-of-view
}
\DeclareAcronym{GNSS}{
  short=GNSS,
  long=global navigation satellite system
}
\DeclareAcronym{GPS}{
  short=GPS,
  long=global positioning system
}
\DeclareAcronym{LIDAR}{
  short=LIDAR,
  long=Light detection and ranging
}
\DeclareAcronym{LOS}{
  short=LOS,
  long=line-of-sight
}
\DeclareAcronym{LPF}{
  short=LPF,
  long=low pass filter
}
\DeclareAcronym{LTE}{
  short=LTE,
  long=long term evolution
}
\DeclareAcronym{LS}{
	short=LS,
	long=least square
}
\DeclareAcronym{MIMO}{
  short=MIMO,
  long=multiple-input multiple-output
}
\DeclareAcronym{mmWave}{
  short=mmWave,
  long=millimeter-wave
}
\DeclareAcronym{MRR}{
  short=MRR,
  long=medium range radar
}
\DeclareAcronym{NLOS}{
  short=NLOS,
  long=non-line-of-sight
}
\DeclareAcronym{NR}{
  short=NR,
  long=new radio
}
\DeclareAcronym{OFDM}{
  short=OFDM,
  long=orthogonal frequency-division multiplexing
}
\DeclareAcronym{ppm}{
  short=ppm,
  long=parts-per-million
}
\DeclareAcronym{RF}{
	short=RF,
	long=radio frequency
}

\DeclareAcronym{RMS}{
  short=RMS,
  long=root-mean-square
}
\DeclareAcronym{RPE}{
  short=RPE,
  long=relative precoding efficiency
}
\DeclareAcronym{RSU}{
  short=RSU,
  long=roadside unit
}

\DeclareAcronym{RX}{
  short=RX,
  long=receiver
}
\DeclareAcronym{SNR}{
  short=SNR,
  long=signal-to-noise ratio
}
\DeclareAcronym{TDoA}{
  short=TDoA,
  long=time difference of arrival
}

\DeclareAcronym{ToA}{
  short=ToA,
  long=time of arrival
}

\DeclareAcronym{TX}{
  short=TX,
  long=transmitter
}

\DeclareAcronym{UL}{
  short=UL,
  long=uplink
}

\DeclareAcronym{ULA}{
  short=ULA,
  long=uniform linear array
}
\DeclareAcronym{URA}{
	short=URA,
	long=uniform rectangular array
}

\DeclareAcronym{V2I}{
  short=V2I,
  long=vehicle-to-infrastructure
}
\DeclareAcronym{V2V}{
  short=V2V,
  long=vehicle-to-vehicle
}
\DeclareAcronym{V2X}{
  short=V2X,
  long=vehicle-to-everything
}
\DeclareAcronym{VRU}{
  short=VRU,
  long=vulnerable road user
}





==> Machine Learning Aided mmWave Vehicular Localization/Other/macros.tex <==
\usepackage{amsmath,amssymb}
% Blackboard capital letters
\newcommand{\bbA}{{\mathbb{A}}}
\newcommand{\bbB}{{\mathbb{B}}}
\newcommand{\bbC}{{\mathbb{C}}}
\newcommand{\bbD}{{\mathbb{D}}}
\newcommand{\bbE}{{\mathbb{E}}}
\newcommand{\bbF}{{\mathbb{F}}}
\newcommand{\bbG}{{\mathbb{G}}}
\newcommand{\bbH}{{\mathbb{H}}}
\newcommand{\bbI}{{\mathbb{I}}}
\newcommand{\bbJ}{{\mathbb{J}}}
\newcommand{\bbK}{{\mathbb{K}}}
\newcommand{\bbL}{{\mathbb{L}}}
\newcommand{\bbM}{{\mathbb{M}}}
\newcommand{\bbN}{{\mathbb{N}}}
\newcommand{\bbO}{{\mathbb{O}}}
\newcommand{\bbP}{{\mathbb{P}}}
\newcommand{\bbQ}{{\mathbb{Q}}}
\newcommand{\bbR}{{\mathbb{R}}}
\newcommand{\bbS}{{\mathbb{S}}}
\newcommand{\bbT}{{\mathbb{T}}}
\newcommand{\bbU}{{\mathbb{U}}}
\newcommand{\bbV}{{\mathbb{V}}}
\newcommand{\bbW}{{\mathbb{W}}}
\newcommand{\bbX}{{\mathbb{X}}}
\newcommand{\bbY}{{\mathbb{Y}}}
\newcommand{\bbZ}{{\mathbb{Z}}}
% Bold lowercase
\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bb}{{\mathbf{b}}}
\newcommand{\bc}{{\mathbf{c}}}
\newcommand{\bd}{{\mathbf{d}}}
\newcommand{\bee}{{\mathbf{e}}}
\newcommand{\bff}{{\mathbf{f}}}
\newcommand{\bg}{{\mathbf{g}}}
\newcommand{\bh}{{\mathbf{h}}}
\newcommand{\bi}{{\mathbf{i}}}
\newcommand{\bj}{{\mathbf{j}}}
\newcommand{\bk}{{\mathbf{k}}}
\newcommand{\bl}{{\mathbf{l}}}
\newcommand{\bmm}{{\mathbf{m}}}
\newcommand{\bn}{{\mathbf{n}}}
\newcommand{\bo}{{\mathbf{o}}}
\newcommand{\bp}{{\mathbf{p}}}
\newcommand{\bq}{{\mathbf{q}}}
\newcommand{\br}{{\mathbf{r}}}
\newcommand{\bs}{{\mathbf{s}}}
\newcommand{\bt}{{\mathbf{t}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bv}{{\mathbf{v}}}
\newcommand{\bw}{{\mathbf{w}}}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\bz}{{\mathbf{z}}}
\newcommand{\bzero}{{\mathbf{0}}}
\newcommand{\bone}{{\mathbf{1}}}
% Bold capital letters
\newcommand{\bA}{{\mathbf{A}}}
\newcommand{\bB}{{\mathbf{B}}}
\newcommand{\bC}{{\mathbf{C}}}
\newcommand{\bD}{{\mathbf{D}}}
\newcommand{\bE}{{\mathbf{E}}}
\newcommand{\bF}{{\mathbf{F}}}
\newcommand{\bG}{{\mathbf{G}}}
\newcommand{\bH}{{\mathbf{H}}}
\newcommand{\bI}{{\mathbf{I}}}
\newcommand{\bJ}{{\mathbf{J}}}
\newcommand{\bK}{{\mathbf{K}}}
\newcommand{\bL}{{\mathbf{L}}}
\newcommand{\bM}{{\mathbf{M}}}
\newcommand{\bN}{{\mathbf{N}}}
\newcommand{\bO}{{\mathbf{O}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\bQ}{{\mathbf{Q}}}
\newcommand{\bR}{{\mathbf{R}}}
\newcommand{\bS}{{\mathbf{S}}}
\newcommand{\bT}{{\mathbf{T}}}
\newcommand{\bU}{{\mathbf{U}}}
\newcommand{\bV}{{\mathbf{V}}}
\newcommand{\bW}{{\mathbf{W}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\bY}{{\mathbf{Y}}}
\newcommand{\bZ}{{\mathbf{Z}}}
% lowercase non-bold letters \mathrm
\newcommand{\rma}{{\mathrm{a}}}
\newcommand{\rmb}{{\mathrm{b}}}
\newcommand{\rmc}{{\mathrm{c}}}
\newcommand{\rmd}{{\mathrm{d}}}
\newcommand{\rme}{{\mathrm{e}}}
\newcommand{\rmf}{{\mathrm{f}}}
\newcommand{\rmg}{{\mathrm{g}}}
\newcommand{\rmh}{{\mathrm{h}}}
\newcommand{\rmi}{{\mathrm{i}}}
\newcommand{\rmj}{{\mathrm{j}}}
\newcommand{\rmk}{{\mathrm{k}}}
\newcommand{\rml}{{\mathrm{l}}}
\newcommand{\rmm}{{\mathrm{m}}}
\newcommand{\rmn}{{\mathrm{n}}}
\newcommand{\rmo}{{\mathrm{o}}}
\newcommand{\rmp}{{\mathrm{p}}}
\newcommand{\rmq}{{\mathrm{q}}}
\newcommand{\rmr}{{\mathrm{r}}}
\newcommand{\rms}{{\mathrm{s}}}
\newcommand{\rmt}{{\mathrm{t}}}
\newcommand{\rmu}{{\mathrm{u}}}
\newcommand{\rmv}{{\mathrm{v}}}
\newcommand{\rmw}{{\mathrm{w}}}
\newcommand{\rmx}{{\mathrm{x}}}
\newcommand{\rmy}{{\mathrm{y}}}
\newcommand{\rmz}{{\mathrm{z}}}
\newcommand{\rmzero}{{\mathrm{0}}}
\newcommand{\rmone}{{\mathrm{1}}}
% uppercase non-bold letters
\newcommand{\rmA}{{\mathrm{A}}}
\newcommand{\rmB}{{\mathrm{B}}}
\newcommand{\rmC}{{\mathrm{C}}}
\newcommand{\rmD}{{\mathrm{D}}}
\newcommand{\rmE}{{\mathrm{E}}}
\newcommand{\rmF}{{\mathrm{F}}}
\newcommand{\rmG}{{\mathrm{G}}}
\newcommand{\rmH}{{\mathrm{H}}}
\newcommand{\rmI}{{\mathrm{I}}}
\newcommand{\rmJ}{{\mathrm{J}}}
\newcommand{\rmK}{{\mathrm{K}}}
\newcommand{\rmL}{{\mathrm{L}}}
\newcommand{\rmM}{{\mathrm{M}}}
\newcommand{\rmN}{{\mathrm{N}}}
\newcommand{\rmO}{{\mathrm{O}}}
\newcommand{\rmP}{{\mathrm{P}}}
\newcommand{\rmQ}{{\mathrm{Q}}}
\newcommand{\rmR}{{\mathrm{R}}}
\newcommand{\rmS}{{\mathrm{S}}}
\newcommand{\rmT}{{\mathrm{T}}}
\newcommand{\rmU}{{\mathrm{U}}}
\newcommand{\rmV}{{\mathrm{V}}}
\newcommand{\rmW}{{\mathrm{W}}}
\newcommand{\rmX}{{\mathrm{X}}}
\newcommand{\rmY}{{\mathrm{Y}}}
\newcommand{\rmZ}{{\mathrm{Z}}}
% Caligraphic capital letters
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
% Bold Caligraphic capital letters
\newcommand{\bcA}{\boldsymbol{\mathcal{A}}}
\newcommand{\bcB}{\boldsymbol{\mathcal{B}}}
\newcommand{\bcC}{\boldsymbol{\mathcal{C}}}
\newcommand{\bcD}{\boldsymbol{\mathcal{D}}}
\newcommand{\bcE}{\boldsymbol{\mathcal{E}}}
\newcommand{\bcF}{\boldsymbol{\mathcal{F}}}
\newcommand{\bcG}{\boldsymbol{\mathcal{G}}}
\newcommand{\bcH}{\boldsymbol{\mathcal{H}}}
\newcommand{\bcI}{\boldsymbol{\mathcal{I}}}
\newcommand{\bcJ}{\boldsymbol{\mathcal{J}}}
\newcommand{\bcK}{\boldsymbol{\mathcal{K}}}
\newcommand{\bcL}{\boldsymbol{\mathcal{L}}}
\newcommand{\bcM}{\boldsymbol{\mathcal{M}}}
\newcommand{\bcN}{\boldsymbol{\mathcal{N}}}
\newcommand{\bcO}{\boldsymbol{\mathcal{O}}}
\newcommand{\bcP}{\boldsymbol{\mathcal{P}}}
\newcommand{\bcQ}{\boldsymbol{\mathcal{Q}}}
\newcommand{\bcR}{\boldsymbol{\mathcal{R}}}
\newcommand{\bcS}{\boldsymbol{\mathcal{S}}}
\newcommand{\bcT}{\boldsymbol{\mathcal{T}}}
\newcommand{\bcU}{\boldsymbol{\mathcal{U}}}
\newcommand{\bcV}{\boldsymbol{\mathcal{V}}}
\newcommand{\bcW}{\boldsymbol{\mathcal{W}}}
\newcommand{\bcX}{\boldsymbol{\mathcal{X}}}
\newcommand{\bcY}{\boldsymbol{\mathcal{Y}}}
\newcommand{\bcZ}{\boldsymbol{\mathcal{Z}}}
% sans serif lowercase
\newcommand{\sfa}{{\mathsf{a}}}
\newcommand{\sfb}{{\mathsf{b}}}
\newcommand{\sfc}{{\mathsf{c}}}
\newcommand{\sfd}{{\mathsf{d}}}
\newcommand{\sfee}{{\mathsf{e}}}
\newcommand{\sfff}{{\mathsf{f}}}
\newcommand{\sfg}{{\mathsf{g}}}
\newcommand{\sfh}{{\mathsf{h}}}
\newcommand{\sfi}{{\mathsf{i}}}
\newcommand{\sfj}{{\mathsf{j}}}
\newcommand{\sfk}{{\mathsf{k}}}
\newcommand{\sfl}{{\mathsf{l}}}
\newcommand{\sfm}{{\mathsf{m}}}
\newcommand{\sfn}{{\mathsf{n}}}
\newcommand{\sfo}{{\mathsf{o}}}
\newcommand{\sfp}{{\mathsf{p}}}
\newcommand{\sfq}{{\mathsf{q}}}
\newcommand{\sfr}{{\mathsf{r}}}
\newcommand{\sfs}{{\mathsf{s}}}
\newcommand{\sft}{{\mathsf{t}}}
\newcommand{\sfu}{{\mathsf{u}}}
\newcommand{\sfv}{{\mathsf{v}}}
\newcommand{\sfw}{{\mathsf{w}}}
\newcommand{\sfx}{{\mathsf{x}}}
\newcommand{\sfy}{{\mathsf{y}}}
\newcommand{\sfz}{{\mathsf{z}}}
\newcommand{\sfzero}{{\mathsf{0}}}
\newcommand{\sfone}{{\mathsf{1}}}
% bold sans serif lowercase
\newcommand{\bsfa}{\boldsymbol{\mathsf{a}}}
\newcommand{\bsfb}{\boldsymbol{\mathsf{b}}}
\newcommand{\bsfc}{\boldsymbol{\mathsf{c}}}
\newcommand{\bsfd}{\boldsymbol{\mathsf{d}}}
\newcommand{\bsfee}{\boldsymbol{\mathsf{e}}}
\newcommand{\bsfff}{\boldsymbol{\mathsf{f}}}
\newcommand{\bsfg}{\boldsymbol{\mathsf{g}}}
\newcommand{\bsfh}{\boldsymbol{\mathsf{h}}}
\newcommand{\bsfi}{\boldsymbol{\mathsf{i}}}
\newcommand{\bsfj}{\boldsymbol{\mathsf{j}}}
\newcommand{\bsfk}{\boldsymbol{\mathsf{k}}}
\newcommand{\bsfl}{\boldsymbol{\mathsf{l}}}
\newcommand{\bsfm}{\boldsymbol{\mathsf{m}}}
\newcommand{\bsfn}{\boldsymbol{\mathsf{n}}}
\newcommand{\bsfo}{\boldsymbol{\mathsf{o}}}
\newcommand{\bsfp}{\boldsymbol{\mathsf{p}}}
\newcommand{\bsfq}{\boldsymbol{\mathsf{q}}}
\newcommand{\bsfr}{\boldsymbol{\mathsf{r}}}
\newcommand{\bsfs}{\boldsymbol{\mathsf{s}}}
\newcommand{\bsft}{\boldsymbol{\mathsf{t}}}
\newcommand{\bsfu}{\boldsymbol{\mathsf{u}}}
\newcommand{\bsfv}{\boldsymbol{\mathsf{v}}}
\newcommand{\bsfw}{\boldsymbol{\mathsf{w}}}
\newcommand{\bsfx}{\boldsymbol{\mathsf{x}}}
\newcommand{\bsfy}{\boldsymbol{\mathsf{y}}}
\newcommand{\bsfz}{\boldsymbol{\mathsf{z}}}
\newcommand{\bsfzero}{\boldsymbol{\mathsf{0}}}
\newcommand{\bsfone}{\boldsymbol{\mathsf{1}}}
% Sans serif capital letters
\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfD}{\mathsf{D}}
\newcommand{\sfE}{\mathsf{E}}
\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\sfI}{\mathsf{I}}
\newcommand{\sfJ}{\mathsf{J}}
\newcommand{\sfK}{\mathsf{K}}
\newcommand{\sfL}{\mathsf{L}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfN}{\mathsf{N}}
\newcommand{\sfO}{\mathsf{O}}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\sfT}{\mathsf{T}}
\newcommand{\sfU}{\mathsf{U}}
\newcommand{\sfV}{\mathsf{V}}
\newcommand{\sfW}{\mathsf{W}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}
% Bold sans serif capital letters
\newcommand{\bsfA}{\boldsymbol{\mathsf{A}}}
\newcommand{\bsfB}{\boldsymbol{\mathsf{B}}}
\newcommand{\bsfC}{\boldsymbol{\mathsf{C}}}
\newcommand{\bsfD}{\boldsymbol{\mathsf{D}}}
\newcommand{\bsfE}{\boldsymbol{\mathsf{E}}}
\newcommand{\bsfF}{\boldsymbol{\mathsf{F}}}
\newcommand{\bsfG}{\boldsymbol{\mathsf{G}}}
\newcommand{\bsfH}{\boldsymbol{\mathsf{H}}}
\newcommand{\bsfI}{\boldsymbol{\mathsf{I}}}
\newcommand{\bsfJ}{\boldsymbol{\mathsf{J}}}
\newcommand{\bsfK}{\boldsymbol{\mathsf{K}}}
\newcommand{\bsfL}{\boldsymbol{\mathsf{L}}}
\newcommand{\bsfM}{\boldsymbol{\mathsf{M}}}
\newcommand{\bsfN}{\boldsymbol{\mathsf{N}}}
\newcommand{\bsfO}{\boldsymbol{\mathsf{O}}}
\newcommand{\bsfP}{\boldsymbol{\mathsf{P}}}
\newcommand{\bsfQ}{\boldsymbol{\mathsf{Q}}}
\newcommand{\bsfR}{\boldsymbol{\mathsf{R}}}
\newcommand{\bsfS}{\boldsymbol{\mathsf{S}}}
\newcommand{\bsfT}{\boldsymbol{\mathsf{T}}}
\newcommand{\bsfU}{\boldsymbol{\mathsf{U}}}
\newcommand{\bsfV}{\boldsymbol{\mathsf{V}}}
\newcommand{\bsfW}{\boldsymbol{\mathsf{W}}}
\newcommand{\bsfX}{\boldsymbol{\mathsf{X}}}
\newcommand{\bsfY}{\boldsymbol{\mathsf{Y}}}
\newcommand{\bsfZ}{\boldsymbol{\mathsf{Z}}}
% Bold greek
% Source: https://www.sharelatex.com/learn/List_of_Greek_letters_and_math_symbols
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bvarepsilon}{\boldsymbol{\varepsilon}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\betae}{\boldsymbol{\eta}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bvartheta}{\boldsymbol{\vartheta}}
\newcommand{\biota}{\boldsymbol{\iota}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\bvarrho}{\boldsymbol{\varrho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bupsilon}{\boldsymbol{\upsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bchi}{\boldsymbol{\chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}
%
% Commonly Used Terms
\newcommand{\transp}{{\sf{T}}}
\newcommand{\compj}{{\rm{j}}}
\newcommand{\tr}{{\rm{tr}}}
\renewcommand{\vec}{{\rm{vec}}}
\newcommand{\diag}{{\rm{diag}}}
\newcommand{\supp}{{\rm{supp}}}
\newcommand{\sinc}{{\rm{sinc}}}

%
% Miscellaneous
\makeatletter
\def\munderbar#1{\underline{\sbox\tw@{$#1$}\dp\tw@\z@\box\tw@}}
\makeatother
%
\newcommand{\dBm}{\SI{}{\decibel}\rmm}











